On stochastic control under Poisson observations: optimality of a barrier strategy in a general L\'evy model

We study a version of the stochastic control problem of minimizing the sum of running and controlling costs, where control opportunities are restricted to independent Poisson arrival times. Under a general setting driven by a general L\'evy process, we show the optimality of a periodic barrier strategy, which moves the process upward to the barrier whenever it is observed to be below it. The convergence of the optimal solutions to those in the continuous-observation case is also shown.

==> style-common.tex <==
%%%%%%    footnote       %%%%%%

\renewcommand{\thefootnote}{(\arabic{footnote})}
%\renewcommand{\thefootnote}{\fnsymbol{footnote}}

\makeatletter
\@addtoreset{footnote}{page}
\makeatother


%%%%%%    enumi       %%%%%%

\usepackage{style-enumitem}

\renewcommand{\theenumi}{\roman{enumi}}
\renewcommand{\labelenumi}{(\theenumi)}
\renewcommand{\theenumii}{\alph{enumii}}
\renewcommand{\labelenumii}{(\theenumi-\theenumii)}


%%%%%%    package       %%%%%%
\usepackage{amsthm}
\usepackage{amsmath,amssymb,latexsym,amsfonts,mathrsfs}

\newcommand{\n}{\nonumber}


%%%%%%    symbols       %%%%%%

\renewcommand{\Re}{\mathop{\rm Re}}
\renewcommand{\Im}{\mathop{\rm Im}}
\newcommand{\Var}{\mathop{\rm Var}}
\newcommand{\Cov}{\mathop{\rm Cov}}
\newcommand{\sgn}{\mathop{\rm sgn}}

\newcommand{\Supp}{\mathop{\rm Supp}}
\newcommand{\tr}{\mathop{\rm tr}}
\newcommand{\Tr}{\mathop{\rm Tr}}
\newcommand{\Det}{\mathop{\rm Det}}
\newcommand{\Log}{\mathop{\rm Log}}

\newcommand{\eps}{\ensuremath{\varepsilon}}

\newcommand{\indep}{\mathop{\rotatebox[origin=a]{90}{$ \models $}}}
\newcommand{\mapsot}{\mathop{\rotatebox[origin=a]{180}{$ \mapsto $}}} 

\newcommand{\law}{\stackrel{{\rm law}}{=}}
\newcommand{\lawto}{\stackrel{{\rm law}}{\longrightarrow}}
\newcommand{\dist}{\stackrel{{\rm d}}{=}}
\newcommand{\dto}{\stackrel{{\rm d}}{\longrightarrow}}
\newcommand{\wto}{\stackrel{{\rm w}}{\longrightarrow}}
\newcommand{\fd}{\stackrel{{\rm f.d.}}{\longrightarrow}}

\newcommand{\tend}[2]{\mathrel{\mathop{\longrightarrow}\limits^{#1}_{#2}}}
\newcommand{\nyoro}[2]{\mathrel{\mathop{\sim}\limits^{#1}_{#2}}}

\renewcommand{\hat}{\widehat}
\renewcommand{\tilde}{\widetilde}
\renewcommand{\bar}{\overline}
\newcommand{\un}[1]{\underline{#1}}
\newcommand{\up}{\ensuremath{\uparrow}}
\newcommand{\down}{\ensuremath{\downarrow}}
\newcommand{\bul}{\ensuremath{\bullet \ }}



%%%%%%    brackets       %%%%%%

\newcommand{\absol}[1]{\left| #1 \right|} %absolute value
\newcommand{\norm}[1]{\left\| #1 \right\|} %norm
\newcommand{\rbra}[1]{\!\left( #1 \right)} %round brackets or parentheses
\newcommand{\cbra}[1]{\!\left\{ #1 \right\}} %curly brackets or braces
\newcommand{\sbra}[1]{\!\left[ #1 \right]} %square brackets or brackets
\newcommand{\abra}[1]{\!\left\langle #1 \right\rangle} %angle brackets or chevrons
\newcommand{\floor}[1]{\!\left\lfloor #1 \right\rfloor \!} %angle brackets or chevrons
\newcommand{\ceil}[1]{\!\left\lceil #1 \right\rceil} %angle brackets or chevrons

\newcommand{\mat}[1]{\begin{matrix} #1 \end{matrix}} % 
\newcommand{\pmat}[1]{\begin{pmatrix} #1 \end{pmatrix}} %()
\newcommand{\vmat}[1]{\begin{vmatrix} #1 \end{vmatrix}} %||
\newcommand{\detmat}[1]{\begin{vmatrix} #1 \end{vmatrix}} %||
\newcommand{\Vmat}[1]{\begin{Vmatrix} #1 \end{Vmatrix}} %\| \|
\newcommand{\bmat}[1]{\begin{bmatrix} #1 \end{bmatrix}} %[]
\newcommand{\Bmat}[1]{\begin{Bmatrix} #1 \end{Bmatrix}} %\{ \}



%%%%%%  capital fonts   %%%%%%

\newcommand{\bA}{\ensuremath{\mathbb{A}}}
\newcommand{\bB}{\ensuremath{\mathbb{B}}}
\newcommand{\bC}{\ensuremath{\mathbb{C}}}
\newcommand{\bD}{\ensuremath{\mathbb{D}}}
\newcommand{\bE}{\ensuremath{\mathbb{E}}}
\newcommand{\bF}{\ensuremath{\mathbb{F}}}
\newcommand{\bG}{\ensuremath{\mathbb{G}}}
\newcommand{\bH}{\ensuremath{\mathbb{H}}}
\newcommand{\bI}{\ensuremath{\mathbb{I}}}
\newcommand{\bJ}{\ensuremath{\mathbb{J}}}
\newcommand{\bK}{\ensuremath{\mathbb{K}}}
\newcommand{\bL}{\ensuremath{\mathbb{L}}}
\newcommand{\bM}{\ensuremath{\mathbb{M}}}
\newcommand{\bN}{\ensuremath{\mathbb{N}}}
\newcommand{\bO}{\ensuremath{\mathbb{O}}}
\newcommand{\bP}{\ensuremath{\mathbb{P}}}
\newcommand{\bQ}{\ensuremath{\mathbb{Q}}}
\newcommand{\bR}{\ensuremath{\mathbb{R}}}
\newcommand{\bS}{\ensuremath{\mathbb{S}}}
\newcommand{\bT}{\ensuremath{\mathbb{T}}}
\newcommand{\bU}{\ensuremath{\mathbb{U}}}
\newcommand{\bV}{\ensuremath{\mathbb{V}}}
\newcommand{\bW}{\ensuremath{\mathbb{W}}}
\newcommand{\bX}{\ensuremath{\mathbb{X}}}
\newcommand{\bY}{\ensuremath{\mathbb{Y}}}
\newcommand{\bZ}{\ensuremath{\mathbb{Z}}}

\newcommand{\cA}{\ensuremath{\mathcal{A}}}
\newcommand{\cB}{\ensuremath{\mathcal{B}}}
\newcommand{\cC}{\ensuremath{\mathcal{C}}}
\newcommand{\cD}{\ensuremath{\mathcal{D}}}
\newcommand{\cE}{\ensuremath{\mathcal{E}}}
\newcommand{\cF}{\ensuremath{\mathcal{F}}}
\newcommand{\cG}{\ensuremath{\mathcal{G}}}
\newcommand{\cH}{\ensuremath{\mathcal{H}}}
\newcommand{\cI}{\ensuremath{\mathcal{I}}}
\newcommand{\cJ}{\ensuremath{\mathcal{J}}}
\newcommand{\cK}{\ensuremath{\mathcal{K}}}
\newcommand{\cL}{\ensuremath{\mathcal{L}}}
\newcommand{\cM}{\ensuremath{\mathcal{M}}}
\newcommand{\cN}{\ensuremath{\mathcal{N}}}
\newcommand{\cO}{\ensuremath{\mathcal{O}}}
\newcommand{\cP}{\ensuremath{\mathcal{P}}}
\newcommand{\cQ}{\ensuremath{\mathcal{Q}}}
\newcommand{\cR}{\ensuremath{\mathcal{R}}}
\newcommand{\cS}{\ensuremath{\mathcal{S}}}
\newcommand{\cT}{\ensuremath{\mathcal{T}}}
\newcommand{\cU}{\ensuremath{\mathcal{U}}}
\newcommand{\cV}{\ensuremath{\mathcal{V}}}
\newcommand{\cW}{\ensuremath{\mathcal{W}}}
\newcommand{\cX}{\ensuremath{\mathcal{X}}}
\newcommand{\cY}{\ensuremath{\mathcal{Y}}}
\newcommand{\cZ}{\ensuremath{\mathcal{Z}}}



==> style-e.tex <==
%%%%%%    theorems      %%%%%%
\theoremstyle{plain}
\newtheorem{Thm}{Theorem}[section]
\newtheorem{Thma}{Theorem}
\renewcommand{\theThma}{\Alph{Thma}}
\newtheorem{Thmb}{Theorem}
\renewcommand{\theThmb}{\arabic{section}.\Alph{Thmb}}
\newtheorem{Lem}[Thm]{Lemma}
\newtheorem{Prop}[Thm]{Proposition}
\newtheorem{Cor}[Thm]{Corollary}
\newtheorem{Conj}[Thm]{Conjecture}
\theoremstyle{definition}
\newtheorem{Ass}[Thm]{Assumption}
\newtheorem{Def}[Thm]{Definition}
\newtheorem{Rem}[Thm]{Remark}
\newtheorem{Ex}[Thm]{Example}

\newcommand{\Proof}[2][Proof]{\begin{proof}[{#1}] #2 \end{proof}}





==> style-j.tex <==
%%%%%%    theorems      %%%%%%
\theoremstyle{definition}
\newtheorem{Thm}{'藝}[section]
\newtheorem{Thma}{'藝}
\renewcommand{\theThma}{\Alph{Thma}}
\newtheorem{Thmb}{'藝}
\renewcommand{\theThmb}{\arabic{section}.\Alph{Thmb}}
\newtheorem{Lem}[Thm]{•â'è}
\newtheorem{Prop}[Thm]{–½'è}
\newtheorem{Cor}[Thm]{Œn}
\newtheorem{Ass}[Thm]{‰¼'è}
\newtheorem{Conj}[Thm]{—\'z}
\newtheorem{Def}[Thm]{'è‹`}
\newtheorem{Rem}[Thm]{'}
\newtheorem{Ex}[Thm]{—á}
\newtheorem{Prob}{–â}[section]
\newcounter{Exami}
\newcommand{\Exam}{\noindent \refstepcounter{Exami} $ \boxed{\arabic{Exami}} $ \ }

\newcommand{\Proof}[2][Ø–¾]{
\begin{proof}[{\bf #1}]
#2
\end{proof}
}
\newcommand{\Solution}[2][‰ð]{
\begin{proof}[{\bf #1}]
#2
\end{proof}
}








==> style-layout-paper.tex <==
%%%%%%    layout        %%%%%%
\setlength\topmargin{0mm}
\setlength\headheight{0mm}
\setlength\headsep{0mm}
\setlength\topskip{0mm}
\setlength\textheight{230mm}
\setlength\footskip{20mm}

\setlength\oddsidemargin{0mm}
\setlength\evensidemargin{0mm}
\setlength\textwidth{160mm}

\setlength\parindent{5mm}
\setlength\parskip{3mm}

\pagestyle{plain}
%\pagestyle{empty}



\numberwithin{equation}{section}



\makeatletter
\renewcommand\section{\@startsection {section}{1}{\z@}%
                                   {-3.5ex \@plus -1ex \@minus -.2ex}%
                                   {2.3ex \@plus.2ex}%
                                   {\normalfont\large\bf}}
                                  %{\normalfont\large\sc}}
\makeatother

\makeatletter
\renewcommand\subsection{\@startsection {subsection}{1}{\z@}%
                                   {-3.5ex \@plus -1ex \@minus -.2ex}%
                                   {2.3ex \@plus.2ex}%
                                   {\normalfont\normalsize\bf}}
                                  %{\normalfont\normalsize\sc}}
\makeatother


